ManyDG: Many-domain Generalization for Healthcare Applications

The vast amount of health data has been continuously collected for each patient, providing opportunities to support diverse healthcare predictive tasks such as seizure detection and hospitalization prediction. Existing models are mostly trained on other patients data and evaluated on new patients. Many of them might suffer from poor generalizability. One key reason can be overfitting due to the unique information related to patient identities and their data collection environments, referred to as patient covariates in the paper. These patient covariates usually do not contribute to predicting the targets but are often difficult to remove. As a result, they can bias the model training process and impede generalization. In healthcare applications, most existing domain generalization methods assume a small number of domains. In this paper, considering the diversity of patient covariates, we propose a new setting by treating each patient as a separate domain (leading to many domains). We develop a new domain generalization method ManyDG, that can scale to such many-domain problems. Our method identifies the patient domain covariates by mutual reconstruction and removes them via an orthogonal projection step. Extensive experiments show that ManyDG can boost the generalization performance on multiple real-world healthcare tasks (e.g., 3.7% Jaccard improvements on MIMIC drug recommendation) and support realistic but challenging settings such as insufficient data and continuous learning.

==> MNIST.tex <==
\subsection{Verifying on benchmark digit classification}
\paragraph{Digit Datasets and Settings} We conduct multi-source digit classification on {\em MNIST} \citep{lecun1998gradient}, {\em MNIST-M} \citep{ganin2015unsupervised}, {\em Street View House Numbers (SVHN)} \citep{netzer2011reading}, {\em USPS} \cite{hull1994database} and {\em SYN Digits} \cite{roy2018effects}. The inputs of all datasets are preprocessed into a similar $3\times 28\times 28$ formats with pixel values in $[0,1]$. Data processing details can be found in Appendix.  We conduct then following experiments:
\begin{itemize}
    \item {\bf Generalization Performance.} Conduct five-fold leave one source out strategy for evaluating the generation performance on another four sources. The results are summarized in Table~\ref{tb:digit_result}, which shows that on average our proposed model is comparable or better than baselines in this task.
    \item {\bf Visualization on Representation Structure.}  We further optimize our model on training sets from all five datasets and evaluate the learned representations from $128\times 5=640$ test images per dataset. We use TSNE \cite{van2008visualizing} for plotting and show the results in Figure~\ref{fig:digit_rep_vis}. We compare the representations from our model (before and after orthogonal projection) to the representations from Base model and color-code each sample by domains and by labels.
\end{itemize}

\begin{table}[!thb]
\centering
\caption{Result Comparison on Digit Classification (\%)}
\resizebox{0.99\textwidth}{!}{\begin{tabular}{c|ccccc|c} 
\toprule 
  \multirow{2}{*}{\bf Models} & 
  {$mt,up,sv,sy$} & {$mm,up,sv,sy$} & {$mm,mt,sv,sy$} & {$mm,mt,up,sy$} & {$mm,mt,up,sv$} & 
  \multirow{2}{*}{Average} \\
  & {$\rightarrow mm$} & {$\rightarrow mt$}
  & {$\rightarrow up$} & {$\rightarrow sv$}
  & {$\rightarrow sy$} & \\
  \midrule
{\bf Base} & 64.12 $\pm$ 0.2564 & 97.44 $\pm$ 0.045 & 90.2 $\pm$ 0.2134 & 45.81 $\pm$ 0.5732 & 47.2 $\pm$ 0.2329 & 68.95 $\pm$ 0.2642 \\
{\bf CondAdv} & 65.62 $\pm$ 0.3047 & 98.33 $\pm$ 0.05005 & 90.66 $\pm$ 0.2561 & 43.57 $\pm$ 0.8804 & 50.38 $\pm$ 0.328 & 69.71 $\pm$ 0.3639 \\
{\bf DANN} & 61.34 $\pm$ 0.2288 & 98.23 $\pm$ 0.02835 & 90.67 $\pm$ 0.2035 & 44.16 $\pm$ 0.636 & 47.39 $\pm$ 0.3704 & 68.36 $\pm$ 0.2934 \\
{\bf IRM} & 62.69 $\pm$ 0.4187 & 97.68 $\pm$ 0.06542 & 88.71 $\pm$ 0.3862 & 44.19 $\pm$ 1.5 & 45.59 $\pm$ 0.8487 & 67.77 $\pm$ 0.6439 \\
{\bf SagNet} & 63.56 $\pm$ 0.1692 & 97.93 $\pm$ 0.03747 & 90.83 $\pm$ 0.1884 & 40.84 $\pm$ 3.023 & 49.24 $\pm$ 0.2468 & 68.48 $\pm$ 0.7329 \\
{\bf PCL} & 61.5 $\pm$ 0.3289 & 98.28 $\pm$ 0.02728 & {\bf 91.01 $\pm$ 0.2065} & 41.28 $\pm$ 0.546 & 49.55 $\pm$ 0.5456 & 68.32 $\pm$ 0.3309 \\
{\bf MLDG} & {\bf 67.48 $\pm$ 0.2559} & 97.29 $\pm$ 0.04821 & 88.16 $\pm$ 0.1817 & {\bf 46.03 $\pm$ 0.2192} & 46.73 $\pm$ 0.3956 & 68.84 $\pm$ 0.2201 \\
\midrule
{\bf \method} & 67.11 $\pm$ 0.278 & {\bf 98.53 $\pm$ 0.02561} & 89.82 $\pm$ 0.09241 & 45.8 $\pm$ 0.2465 & {\bf 50.54 $\pm$ 0.4329} & {\bf 70.36 $\pm$ 0.2151} \\
\bottomrule
\multicolumn{7}{c}{* $mt$ stands for MNIST, $mm$ stands for MNIST-M, $up$ stands for USPS, $sv$ standard for SVHN, $sy$ stands for SYN Digits.}
\end{tabular}}
\label{tb:digit_result} 
\end{table}

\begin{figure*}[!tbp]
	\centering
    \includegraphics[width=13.1cm]{fig/digit_rep.png}
	\caption{Representation Structure on Digit Classification}
	\label{fig:digit_rep_vis}
\end{figure*}


==> experiment_bak.tex <==
\section{Experiments}
We evaluate our model on various experimental settings and 

\subsection{Covariate-Shifted MNIST}
This is a benchmark hand written digit dataset, containing 50,000 training images and 10,000 test images. Digits froom 0 to 9 have roughly 5,000 samples each in the training test and 1,000 each in the test set. Any simple CNN model can easily achieve 99\% accuracy on the original dataset. We choose a two-layer CNN model as the backbone model with batch normalization layer, ReLU layer and 2D maxpooling layers after each 2D convolution layer. As the final layer, we flatten the features and add a linear layer for predictor. This model achieves 99\% accuracy stably.

To MIMIC the covariate shift, we use sine and cosine encodings (used in positional encoding) to add noise for images. As shown in the figure below.

\begin{figure*}[!htbp]
	\centering
	\begin{minipage}[t]{0.25\textwidth}
    \centering
    \includegraphics[width=3cm]{fig/noise.png}
    \end{minipage}
	\begin{minipage}[t]{0.74\textwidth}
    \centering
    \includegraphics[width=9cm]{fig/digits_example.png}
    \end{minipage}
	\label{fig:MNIST}
	\caption{Sine and Cosine Encoding Modularized MNIST}
\end{figure*}

We consider the following covariate-shift senarios and compared the accuracy performance between the CNN model and our \method with the same backbone. Two models has exactly the same other settings, such as $0.001$ as the learning rate.
\begin{itemize}
    \item \textbf{Original MNIST data}. We does not change the data.
    \item \textbf{Covariate-shift for All.} We randomly select cosine and sine waves from the noisy matrix and apply to all training and test samples.
    \item \textbf{Opposite Stepped Covariate-Shift.} In training, the covariate shift is added for 0\% label-0 data, 10\% label-1 data, 20\% label-2 data... In test, the covariate shift is added for 90\% label-0 data, 80\% label-1 data, 70\% label-2 data...
    \item \textbf{Stepped Covariate-Shift.} In training, the covariate shift is added for 0\% label-0 data, 10\% label-1 data, 20\% label-2 data... In test, the covariate shift is added for 0\% label-0 data, 10\% label-1 data, 20\% label-2 data...
    \item \textbf{50\% Covariate Shift for All.} Add covariate shift for 50\% of the data per label, for both training and test.
    \item \textbf{Random Covariate Shift.} Select random proportion of data to add covariate shift, separately for training and test.
    \item \textbf{Covariate Shift for Training Only}. We add covariate shift for all training data.
    \item \textbf{Covariate Shift for Test Only.} We add covariate shift for all test data only.
\end{itemize}

\begin{table}[h!]
\centering
\caption{Comparison between CNN model and \method on Covariate-shifted MNIST}
\begin{tabular}{c|cc} 
\toprule 
  {\bf Scenario} & {\bf CNN Model (\%)} & {\bf \method (\%)} \\
  \midrule
  Original MNIST & 99.28 $\pm$ 0.05 & 99.22 $\pm$ 0.04 \\
  Covariate-shift for All & 98.32 $\pm$ 0.25 & 98.42 $\pm$ 0.11 \\
  Opposite Stepped Covariate-Shft & 69.36 $\pm$ 2.32 & 95.57 $\pm$ 1.09 \\
  Stepped Covariate-Shft & 70.63 $\pm$ 1.78 & 98.50 $\pm$ 0.30 \\
  50\% Covariate Shift for All & 84.61 $\pm$ 0.73 & 98.49 $\pm$ 0.21 \\
  Random Covaraite Shift & 61.27 $\pm$ 2.11 & 96.42 $\pm$ 0.10 \\
  Covariate Shift for Training Only & 93.17 $\pm$ 0.10 & 96.69 $\pm$ 0.53 \\
  Covariate Shift for Test Only & 31.54 $\pm$ 3.58 & 38.37 $\pm$ 2.19 \\
\bottomrule
\end{tabular} \label{tb:MNIST} 
\end{table}

\subsection{MNIST and MNIST-M}
MNIST-M is created by combining MNIST digits with the patches randomly extracted from color photos of BSDS500 as their background. It contains 59,001 training and 90,001 test images.

\begin{table}[h!]
\centering
\caption{Comparison between CNN model and \method on Covariate-shifted MNIST}
\begin{tabular}{c|cc} 
\toprule 
  {\bf Scenario} & {\bf CNN Model (\%)} & {\bf \method (\%)} \\
  \midrule
  MNIST-M \textbf{as training}, MNIST \textbf{as test} & 95.44 $\pm$ 0.55 & 97.29 $\pm$ 0.37 \\
  MNIST \textbf{as training}, MNIST-M \textbf{as test} & 19.44 $\pm$ 0.23 & 15.87 $\pm$ 1.27 \\
  MNIST-M train + MNIST train \textbf{as training} & 91.86 $\pm$ 0.44 & 93.43 $\pm$ 0.13 \\
  MNIST-M test + MNIST train \textbf{as training} & 83.79 $\pm$ 0.54 & 85.13 $\pm$ 0.17 \\
  MNIST-M train + MNIST test \textbf{as training} & 73.94 $\pm$ 0.23 & 96.72 $\pm$ 0.21 \\
\bottomrule
\end{tabular} \label{tb:MNIST} 
\end{table}

\subsection{Multiple-domain dataset: DomainNet}
Add experiments here.


\subsection{EEG IIIC Seizure Detection Task}
\paragraph{Data Description.} This is the EEG seizure data provided by MGH with over 3000 patients. We have 134,203 train samples, 18,034 val samples, 13,072 test samples. Each signal is a 16-channel signal and we conduct 6-class classification. We remove out the signals that have fewer than 5 expert votes. The following experiments are done with 3 random splits. All model uses the same backbone.


\begin{table}[h!]
\centering
\caption{Performance on EEG IIIC seizure}
\begin{tabular}{c|ccc} 
\toprule 
  {\bf Scenario} & {\bf CNN Model (\%)} & {\bf \method (\%)} & {\bf \method+OOD (\%)} \\
  \midrule
  All data & 65.13 $\pm$ 0.44 & 66.85 $\pm$ 0.50 & 67.32 $\pm$ 1.10 \\
  Mid-scale data (1000 patients data) & 50.64 $\pm$ 2.39 & 55.28 $\pm$ 2.53 & 56.06 $\pm$ 2.37 \\
  Small data (200 patients data) & 33.75 $\pm$ 4.60 & 50.32 $\pm$ 5.18 & 50.68 $\pm$ 5.75 \\
\bottomrule
\end{tabular} \label{tb:Seizure} 
\end{table}


\subsection{EEG Sleep Staging Task}
We use the open sleep EDF dataset for the experiments. In the sleep edf datasets, there are in total 78 patients and we split 62 patients into training set, 8 patients into validation set and the remaining 8 patients into test set. In total, the training, validation and test set has 328,258, 43,424, 43,407 data points. We compare the two models in different scenarios with varying amount of training data.

\begin{table}[h!]
\centering
\caption{Performance on EEG IIIC seizure}
\begin{tabular}{c|cc} 
\toprule 
  {\bf Scenario} & {\bf CNN Model (\%)} & {\bf \method (\%)} \\
  \midrule
  Full data per patient & 89.50 $\pm$ 0.33 & 90.34 $\pm$ 0.12\\
  300 data points per patient & 88.66 $\pm$ 0.25 & 89.51 $\pm$ 0.17 \\
  100 data points per patient & 86.33 $\pm$ 0.72 & 87.76 $\pm$ 0.45 \\
  20 data points per patient & 79.40 $\pm$ 0.30 & 81.66 $\pm$ 0.68 \\
\bottomrule
\end{tabular} \label{tb:Seizure} 
\end{table}

\subsection{MIMIC-III Drug Recommendation Task}
This task is to predict the medication set for each patient hospital visit. The setting follows GAMENet, SafeDrug, RETAIN.

\begin{table}[h!]
\centering
\caption{Performance on MIMIC-III Drug Recommendation}
\begin{tabular}{c|cccc} 
\toprule 
  {\bf Model} & {\bf DDI} & {\bf Jaccard} & {\bf AUC-PR} & {\bf F1} \\
  \midrule
  RETAIN & 0.07849 $\pm$ 0.00122 & 0.4735 $\pm$ 0.002203 & 0.7551 $\pm$ 0.0005953 & 0.6353 $\pm$ 0.001986\\
  GAMENet & 0.08884 $\pm$ 0.0006711 & 0.4818 $\pm$ 0.0009994 & 0.7397 $\pm$ 0.000966 & 0.6411 $\pm$ 0.0009816 \\
  SafeDrug & 0.0675 $\pm$ 0.001943 & 0.507 $\pm$ 0.0001914 & 0.7593 $\pm$ 0.000348 & 0.6642 $\pm$ 0.0002096 \\
  RETAIN-\method & 0.07912 $\pm$ 0.0009301 & 0.4967 $\pm$ 0.0009427 & 0.7496 $\pm$ 0.002029 & 0.6552 $\pm$ 0.000762 \\
  GAMENet-\method & 0.07976 $\pm$ 0.0009867 & 0.5134 $\pm$ 0.00136 & 0.7639 $\pm$ 0.0007384 & 0.6694 $\pm$ 0.001303 \\
  SafeDrug-\method & 0.06343 $\pm$ 0.001409 & 0.5171 $\pm$ 0.001107 & 0.766 $\pm$ 0.0009764 & 0.6728 $\pm$ 0.001044\\
\bottomrule
\end{tabular} \label{tb:Seizure} 
\end{table}



